Masking Gaussian Elimination at Arbitrary Order, with Application to Multivariate- and Code-Based PQC

Digital signature schemes based on multivariate- and code-based hard problems are promising alternatives for lattice-based signature schemes, due to their small signature size. Gaussian Elimination (GE) is a critical operation in the signing procedure of these schemes. In this paper, we provide a masking scheme for GE with back substitution to defend against first- and higher-order attacks. To the best of our knowledge, this work is the first to analyze and propose masking techniques for multivariate- or code-based DS algorithms. We propose a masked algorithm for transforming a system of linear equations into row-echelon form. This is realized by introducing techniques for efficiently making leading (pivot) elements one while avoiding costly conversions between Boolean and multiplicative masking at all orders. We also propose a technique for efficient masked back substitution, which eventually enables a secure unmasking of the public output. All novel gadgets are proven secure in the $t$-probing model. Additionally, we evaluate the overhead of our countermeasure for several post-quantum candidates and their different security levels at first-, second-, and third-order, including UOV, MAYO, SNOVA, QR-UOV, and MQ-Sign. Notably, the operational cost of first-, second-, and third-order masked GE is 2.3$\times$ higher, and the randomness cost is 1.2$\times$ higher in MAYO compared to UOV for security levels III and V. In contrast, these costs are similar in UOV and MAYO for one version of level I. We also show detailed performance results for masked GE implementations for all three security versions of UOV on the Arm Cortex-M4 and compare them with unmasked results. Our masked implementation targeting UOV parameters has an overhead of factor 15.1$\times$, 15.2$\times$, and 15.4$\times$ compared to the unprotected implementation for NIST security level I, III, and V.

==> images/nistuov.tex <==
\begin{figure}[ht]
\fbox{\begin{varwidth}{\textwidth}
\begin{subfigure}[t]{0.5\textwidth}
    \begin{small}
    \raggedright 
    $\mathtt{CompactKeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $seed_{sk} \leftarrow \{0, 1\}^{sk\_seed\_len}$
        \item $seed_{pk} \leftarrow \{0, 1\}^{pk\_seed\_len}$
        \item $\pmb{O} := \mathtt{Expand}_{sk}(seed_{sk})$
        \item $\left\{\pmb{P}_i^{(1)}, \pmb{P}_i^{(2)}\right\}_{i \in [m]} := \mathtt{Expand}_{\pmb{P}}(seed_{pk})$
        \item \textbf{for} $i = 1$ upto $m$ \textbf{do}
        \item \quad $\pmb{P}_i^{(3)} := \mathtt{Upper}\left(- \pmb{O}^T \pmb{P}_i^{(1)}\pmb{O} - \pmb{O}^T\pmb{P}_i^{(2)}\right)$
        \item $cpk := \left(seed_{pk}, \left\{\pmb{P}_i^{(3)}\right\}_{i \in [m]}\right)$
        \item $csk := (seed_{pk}, seed_{sk})$
        \item \textbf{return} $(cpk, csk)$
    \end{enumerate}
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{0.5\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{ExpandSK} (csk)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{O} := \mathtt{Expand}_{sk}(seed_{sk})$
        \item $\left\{\pmb{P}_i^{(1)}, \pmb{P}_i^{(2)}\right\}_{i \in [m]} := \mathtt{Expand}_{\pmb{P}}(seed_{pk})$
        \item \textbf{for} $i = 1$ upto $m$ \textbf{do}
        \item \quad $\pmb{S}_i := \left(\pmb{P}_i^{(1)} + \pmb{P}_i^{(1)T}\right)\pmb{O} + \pmb{P}_i^{(2)}$
        \item $esk := \left(seed_{sk}, \pmb{O}, \left\{\pmb{P}_i^{(1)}, \pmb{S}_i\right\}_{i \in [m]}\right)$
       \item \textbf{return} $esk$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{0.5\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Sign} (esk, \mu)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $salt \leftarrow \{0, 1\}^{salt\_len}$
        \item $\pmb{t} := \mathtt{Hash}(\mu || salt)$
        \item \textbf{for} $ctr = 0$ upto $255$ \textbf{do}
        \item \quad $\pmb{v} := \mathtt{Expand}_{\pmb{v}}(\mu || salt || seed_{sk} || ctr)$
        \item \quad $\pmb{L} := \pmb{0}_{m \times m}$
        \item \quad \textbf{for} $i = 1$ upto $m$ \textbf{do}
        \item \quad \quad Set $i$-th row of $\pmb{L}$ to $\pmb{v}^T\pmb{S}_i$
        \item \quad $\pmb{y} := [\pmb{v}^T\pmb{P}_i^{(1)}\pmb{v}]_{i \in [m]}$
        \item \quad $\pmb{x} := \pmb{L}^{-1} (\pmb{t} - \pmb{y})$ // $\pmb{x} = \perp$ if $\det \pmb{L} = 0$
        \item \quad \textbf{if} $\pmb{x} \neq \perp$ \textbf{then}
        \item \quad \quad $\pmb{s} := \begin{bmatrix} \pmb{v} \\ \pmb{0}_m \end{bmatrix} + \begin{bmatrix} \pmb{O} \\ \pmb{I}_m \end{bmatrix} \pmb{x}$
        \item \quad \quad $\sigma := (\pmb{s}, salt)$
        \item \quad \quad \textbf{return} $\sigma$
        \item \textbf{return} $\perp$ 
    \end{enumerate} 
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{0.47\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{ExpandPK} (cpk)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\left\{\pmb{P}_i^{(1)}, \pmb{P}_i^{(2)}\right\}_{i \in [m]} := \mathtt{Expand}_{\pmb{P}}(seed_{pk})$
        \item \textbf{for} $i = 1$ upto $m$ \textbf{do}
        \item \quad $\pmb{P}_i = \begin{bmatrix}
                                 \pmb{P}_i^{(1)} & \pmb{P}_i^{(2)}\\
                                 \pmb{0}         & \pmb{P}_i^{(3)}
                                 \end{bmatrix}$
        \item $epk := \{\pmb{P}_i\}_{i \in [m]}$
        \item \textbf{return} $epk$ 
    \end{enumerate} 
    \end{small}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Verify} (epk, \mu, \sigma = (\pmb{s}, salt))$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{t} := \mathtt{Hash}(\mu || salt)$
        \item \textbf{return} $\pmb{t} == [\pmb{s}^T\pmb{P}_i\pmb{s}]_{i \in [m]}$ 
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{The algorithms of NIST submission UOV \cite{beullensuov}}
\label{fig:nistuov}
% \vspace{-10pt}
\end{figure}

==> images/originaluov.tex <==
\begin{figure}[ht]
\fbox{\begin{varwidth}{\textwidth}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright 
    $\mathtt{KeyGen} ()$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item Pick $m$ uniformly random OV-polynomials $f_1, \ldots , f_m$
        \item $\mathcal{F} := (f_1, \ldots , f_m)$
        \item Pick a uniformly random invertible linear transformation $\mathcal{T} : \mathbb{F}_q^n \rightarrow \mathbb{F}_q^n$
        \item $\mathcal{P} := \mathcal{F} \circ \mathcal{T}$
        \item $pk := \mathcal{P}$
        \item $sk := (\mathcal{F}, \mathcal{T})$
        \item \textbf{return} $(pk, sk)$
    \end{enumerate}
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Sign} (sk = (\mathcal{F}, \mathcal{T}), \mu \in \{0, 1\}^*)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{t} := \mathtt{Hash}(\mu)$
        \item Pick a random preimage $\pmb{u} \in \mathbf{F}_q^n$ of $\pmb{t}$ such that $\mathcal{F}(\pmb{u}) = \pmb{t}$
        \item $\pmb{s} := \mathcal{T}^{-1}(\pmb{u})$
        \item $\sigma := \pmb{s}$
        \item \textbf{return} $\sigma$
    \end{enumerate} 
    \end{small}
    \vspace{3mm}
\end{subfigure}
\begin{subfigure}[t]{\textwidth}
    \begin{small}
    \raggedright
    $\mathtt{Verify} (pk = \mathcal{P}, \mu, \sigma)$
    \begin{enumerate}[wide=0em, itemsep=0pt, parsep=0pt, font=\scriptsize\tt\color{gray}]
        \item $\pmb{t} := \mathtt{Hash}(\mu)$
        \item \textbf{return} $\pmb{t} == \mathcal{P}(\sigma)$
    \end{enumerate} 
    \end{small}
\end{subfigure}
\end{varwidth}}
\caption{The algorithms of original UOV \cite{kipnis1999unbalanced}}
\label{fig:originaluov}
% \vspace{-10pt}
\end{figure}

==> sections/sensitivity.tex <==
%This section contains a detailed discussion on the sensitivity analysis. This analysis  point out those 

\section{Sensitivity Analysis}

We analyze the sensitivity of all the variables and algorithms of the UOV scheme. All public data, including (compact/expanded) public key, message and signature of a message, are non-sensitive. Note that $seed_{pk}$ in the compact representation of the secret key $csk$, $\left\{\pmb{P}_i^{(1)}\right\}_{i \in [m]}$ in the expanded representation of secret key $esk$ are part of the public key, so non-sensitive; the remaining variables in the (compact/expanded) secret key, i.e., $seed_{sk}, \pmb{O}, \left\{\pmb{S}_i\right\}_{i \in [m]}$ are sensitive. Since public key expansion and verification do not manipulate sensitive data, those algorithms are non-sensitive. The remaining algorithms, i.e., compact key generation, secret key expansion, and signature generation, deal with sensitive data; we depict colour-coded diagrams of those algorithms in Fig. \ref{fig:compact_keygen} - \ref{fig:sign}, where red (resp. blue) denotes sensitive (resp. non-sensitive) variables or operations. Next, we discuss the sensitive variables (apart from the public-secret key pair) of the preceding algorithms in more detail.

\subsection{Compact Key Generation and Secret Key Expansion}

In compact key generation and secret key expansion, $\left\{\pmb{P}_i^{(1)}, \pmb{P}_i^{(2)}\right\}_{i \in [m]}$ are only variables that are not part of the compact public-secret key pair $(cpk, csk)$ or expended secret key $esk$, but part of expended public key $epk$, so those variables are non-sensitive. 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{images/compact_keygen.jpg}
\caption{Graphical representation of the compact key generation. Output: $cpk = \left(seed_{pk}, \left\{\pmb{P}_i^{(3)}\right\}_{i \in [m]}\right), csk = (seed_{pk}, seed_{sk})$. {\color{red} Red}: Sensitive, {\color{blue} Blue}: Non-sensitive.}
\label{fig:compact_keygen}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{images/expand_sk.jpg}
\caption{Graphical representation of the expand secret key. Input: $csk = (seed_{pk}, seed_{sk})$. Output: $esk = \left(seed_{sk}, \pmb{O}, \left\{\pmb{P}_i^{(1)}, \pmb{S}_i\right\}_{i \in [m]}\right)$. {\color{red} Red}: Sensitive, {\color{blue} Blue}: Non-sensitive.}
\label{fig:expand_sk}
\end{figure}

\subsection{Signature Generation}

In the signature generation, $\pmb{t}$ is the hash of a message $\mu$ and $salt$, part of signature $\sigma$, so non-sensitive. Pébereau \cite{Pébereau2023one} shows one vector from secret oil space is enough for a key recovery attack. If $\pmb{v}$ is known, $\pmb{s} - \begin{bmatrix} \pmb{v} \\ \pmb{0}_m \end{bmatrix}$, an oil vector, is also known. So, $\pmb{v}$ is sensitive. If $\pmb{L}$ is known, $\pmb{y} = \pmb{t} - \pmb{L}\pmb{x}$ is also known. If $\pmb{y}$ is known, we can recover $\pmb{v}$ by solving $\pmb{z}^T\pmb{P}_i^{(1)}\pmb{z} = \pmb{y}$, that reduce security level. So, $\pmb{L}$ and $\pmb{y}$ are sensitive. Due to the structure of the secret oil space,  $\pmb{x}$, the linear coefficients of the oil vector in $\pmb{s}$ is leaked. So, we consider $\pmb{x}$ as non-sensitive. Based on checking the invertibility of $\pmb{L}$, the timing attack is not an issue as we discard all previous variables if not invertible. The execution time of signature generation leaks $ctr$ value, so we can consider $ctr$ is also non-sensitive.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth]{images/sign.jpg}
\caption{Graphical representation of the Signature. Input: $esk = \left(seed_{sk}, \pmb{O}, \left\{\pmb{P}_i^{(1)}, \pmb{S}_i\right\}_{i \in [m]}\right), \mu$. Output: $\sigma = (\pmb{s}, salt)$. {\color{red} Red}: Sensitive, {\color{blue} Blue}: Non-sensitive.}
\label{fig:sign}
\end{figure}

